Text-driven Visual Synthesis with Latent Diffusion Prior

There has been tremendous progress in large-scale text-to-image synthesis driven by diffusion models enabling versatile downstream applications such as 3D object synthesis from texts, image editing, and customized generation. We present a generic approach using latent diffusion models as powerful image priors for various visual synthesis tasks. Existing methods that utilize such priors fail to use these models' full capabilities. To improve this, our core ideas are 1) a feature matching loss between features from different layers of the decoder to provide detailed guidance and 2) a KL divergence loss to regularize the predicted latent features and stabilize the training. We demonstrate the efficacy of our approach on three different applications, text-to-3D, StyleGAN adaptation, and layered image editing. Extensive results show our method compares favorably against baselines.

==> figures/fig_3D.tex <==
\begin{figure*}[t]
\centering

\mpage{0.48}{{{\small{Jacobian NeRF}}}}\hfill
\mpage{0.48}{{{\small{Ours}}}}\hfill \\

\vspace{1mm}

\mpage{0.01}{\raisebox{0pt}{\rotatebox{90}{\small{jug\footnotemark}}}}  \hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0cm 0cm 0cm 0cm, clip]{images/text/supp/vase_jaco_base1.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0cm 0cm 0cm 0cm, clip]{images/text/supp/vase_jaco_base2.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/vase_jaco_base3.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/vase_jaco_our1.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/vase_jaco_our2.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/vase_jaco_our3.png}}}\\

\vspace{1mm}

\mpage{0.01}{\raisebox{0pt}{\rotatebox{90}{\small{fish\footnotemark}}}}  \hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0cm 0cm 0cm 0cm, clip]{images/text/supp/bird_jaco_base1.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/bird_jaco_base2.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/bird_jaco_base3.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/bird_jaco_our1.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/bird_jaco_our2.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/bird_jaco_our3.png}}}\\

\vspace{1mm}

\mpage{0.01}{\raisebox{0pt}{\rotatebox{90}{\small{blue jug\footnotemark}}}}  \hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0cm 0cm 0cm 0cm, clip]{images/text/supp/boat_jaco_base1.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0cm 0cm 0cm 0cm, clip]{images/text/supp/boat_jaco_base2.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/boat_jaco_base3.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0cm 0cm 0cm 0cm, clip]{images/text/supp/boat_jaco_our1.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/boat_jaco_our2.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0.5cm 0 0.5cm 1cm, clip]{images/text/supp/boat_jaco_our3.png}}}\\

\vspace{1mm}

% \mpage{0.015}{{{\small{\!}}}}\hfill
% \mpage{0.152}{{{\small{CLIP-Mesh~\cite{khalid2022clipmesh}}}}}\hfill
% \mpage{0.152}{{{\small{DreamField~\cite{jain2021dreamfields}}}}}\hfill
% \mpage{0.152}{{{\small{Latent NeRF~\cite{metzer2022latent}}}}}\hfill
% \mpage{0.152}{{{\small{{Ours (Latent NeRF)}}}}}\hfill
% \mpage{0.152}{{{\small{Jocobian NeRF~\cite{sjc}}}}}\hfill
% \mpage{0.152}{{{\small{{Ours (Jocobian NeRF)}}}}}\\


\caption{\textbf{Comparisons on Text-to-3D.} We show a comparison of our approach with Jocobian NeRF~\cite{sjc} in three different viewing point.
}
\vspace{-3mm}
\label{fig:supp_3D}
\end{figure*}

\footnotetext[1]{``A blue jug in a garden filled with mud.''} 
\footnotetext[2]{``A high quality photo of a large blue bird, highly detailed.''} 
\footnotetext[3]{``An inflatable raft that has its top open and a person sitting in it.''} 

==> figures/fig_3D2.tex <==
\begin{figure*}[t]
\centering

\mpage{0.48}{{{\small{Latent NeRF}}}}\hfill
\mpage{0.48}{{{\small{Our}}}}\hfill \\

\mpage{0.01}{\raisebox{0pt}{\rotatebox{90}{\small{jug\footnotemark}}}}  \hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0cm 0cm 0cm 0cm, clip]{images/text/supp/vase_latent_base1.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0cm 0cm 0cm 0cm, clip]{images/text/supp/vase_latent_base2.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/vase_latent_base3.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/vase_latent_our1.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/vase_latent_our2.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/vase_latent_our3.png}}}\\

\vspace{1mm}

\mpage{0.01}{\raisebox{0pt}{\rotatebox{90}{\small{fish\footnotemark}}}}  \hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0cm 0cm 0cm 0cm, clip]{images/text/supp/lego_latent_base1.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/lego_latent_base2.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/lego_latent_base3.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/lego_latent_our1.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/lego_latent_our2.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/lego_latent_our3.png}}}\\

\vspace{1mm}

\mpage{0.01}{\raisebox{0pt}{\rotatebox{90}{\small{blue jug\footnotemark}}}}  \hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0cm 0cm 0cm 0cm, clip]{images/text/supp/ice1.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0cm 0cm 0cm 0cm, clip]{images/text/supp/ice2.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/ice3.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0cm 0cm 0cm 0cm, clip]{images/text/supp/ice_our.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/text/supp/ice_our2.png}}}\hfill
\mpage{0.152}{\frame{\includegraphics[width=\linewidth, trim=0.5cm 0 0.5cm 1cm, clip]{images/text/supp/ice_our3.png}}}\\

\vspace{1mm}

% \mpage{0.015}{{{\small{\!}}}}\hfill
% \mpage{0.152}{{{\small{CLIP-Mesh~\cite{khalid2022clipmesh}}}}}\hfill
% \mpage{0.155}{{{\small{DreamField~\cite{jain2021dreamfields}}}}}\hfill
% \mpage{0.155}{{{\small{Latent NeRF~\cite{metzer2022latent}}}}}\hfill
% \mpage{0.155}{{{\small{{Ours (Latent NeRF)}}}}}\hfill
% \mpage{0.155}{{{\small{Jocobian NeRF~\cite{sjc}}}}}\hfill
% \mpage{0.155}{{{\small{{Ours (Jocobian NeRF)}}}}}\\


\caption{\textbf{Comparisons on Text-to-3D.} We show a comparison of our approach with Latent NeRF~\cite{metzer2022latent} in three different viewing point.
}
\vspace{-3mm}
\label{fig:supp_3D2}
\end{figure*}

\footnotetext[1]{``A blue jug in a garden filled with mud.''} 
\footnotetext[2]{``A lego man.''} 
\footnotetext[3]{``A high quality photo of an ice cream sundae.''} 

==> figures/fig_motivation.tex <==
\begin{figure}[t]
\mfigure{0.48}{images/low_res.pdf} \hfill
\mfigure{0.48}{images/high_res.pdf} \\
\mpage{0.48}{(a) Low-res loss} \hfill
\mpage{0.48}{(b) MLFML (Ours)}\\
\caption{\textbf{Multi-level feature matching loss.}
%
In addition to the \emph{low-resolution} loss~\cite{poole2022dreamfusion}, we introduce a multi-level feature matching loss.
% To generate a high-resolution 3D model, an encoder first takes the generated high-resolution image from StableDiffusion as the input, and produces a latent code $v$.
Like the \emph{low-resolution} loss, $v$ is then perturbed by Gaussian noise and fed into the pretrained UNet of latent stable diffusion to generate a predicted noise $\hat{\epsilon}$.
Instead of directly backpropagating the error $||\epsilon - \hat{\epsilon}||$, we add the error to $v$, and then feed both $v$ and $v + \epsilon - \hat{\epsilon}$ into the decoder. 
We compute the layer-wise feature difference $||G^{l}_{\phi_{dec}}(v)-G^{l}_{\phi_{dec}}(v + \epsilon - \hat{\epsilon})||$ and then backpropagate it.
\\
\yaochih{Distinguish the difference between ``image diffusion'' (a) and ``latent diffusion'' (b)?}
}

\label{fig:motivation}
\end{figure}


==> figures/fig_qualitative_layered.tex <==
\begin{figure*}[t]
\centering
\mpage{0.3}{\includegraphics[width=\linewidth, trim=0 7cm 0 0, clip]{images/placeholder.jpg}}\hfill
\mpage{0.3}{\includegraphics[width=\linewidth, trim=0 7cm 0 0, clip]{images/placeholder.jpg}}\hfill
\mpage{0.3}{\includegraphics[width=\linewidth, trim=0 7cm 0 0, clip]{images/placeholder.jpg}}\\

\vspace{1mm}

\mpage{0.3}{{{\small{Baseline}}}}\hfill
\mpage{0.3}{{{\small{Text2LIVE~\cite{bar2022text2live}}}}}\hfill
\mpage{0.3}{{{\small{\textbf{Ours}}}}}\\

\caption{\textbf{User Study}

}

\label{fig:qualitative_layered}
\end{figure*}

==> tables/ablation_gan.tex <==
\begin{table}[htbp]
  \centering
  % \scriptsize
  % CLIP and LPIPS score of animal experiments. 
  % \vspace{-3mm}
  \caption{We conduct an ablation study using different combinations of losses on StyleGAN Adaptation. CLIP score is computed on generated samples and input text prompts to examine the text-image similarity. LPIPS is computed between all possible pairs in the generated samples to evaluate the diversity of images. $L_{LSD}+L_{KL}+L_{FM}$ refers to the full model.
  }
  \vspace{3mm}
  \resizebox{0.5\columnwidth}{!}{%
    \begin{tabular}{lrrrrrr}
    \toprule
          & \multicolumn{2}{c}{$L_{LSD}+L_{KL}$} & \multicolumn{2}{c}{$L_{LSD}+L_{FM}$} & \multicolumn{2}{c}{$L_{LSD}+L_{KL}+L_{FM}$} \\
          \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
    % \midrule
          Cat $\rightarrow$ & \multicolumn{1}{l}{CLIP$\uparrow$} & \multicolumn{1}{l}{LPIPS$\uparrow$} & \multicolumn{1}{l}{CLIP$\uparrow$} & \multicolumn{1}{l}{LPIPS$\uparrow$} & \multicolumn{1}{l}{CLIP$\uparrow$} & \multicolumn{1}{l}{LPIPS$\uparrow$} \\
    \midrule
    \emojidog~Dog    &   0.288    &  0.594    &   0.288    &  0.582      &   \textbf{0.289}    & \textbf{0.594}\\
    \emojihamster~Hamster   &   \textbf{0.334}   &  0.555   &   {0.330}    &  0.540      &   0.329    &   \textbf{0.569} \\
    \emojibadger~Badger  &   \textbf{0.313}    &  0.537    &   {0.292}    &  0.435       &   0.297    &   \textbf{0.555}\\
    \emojifox~Fox   &   \textbf{0.321}    &  \textbf{0.550}    & { 0.319}     &   0.527      &   0.318    &   0.536 \\
    \emojiotter~Otter   &   0.321    &  0.542   &   \textbf{0.323}    &   0.533      &  0.317     &   \textbf{0.542}\\
    \emojilion~Lion    &  \textbf{0.305}     &   {0.553}   &  0.302     &   0.550    &    {0.302}   &   \textbf{0.555}\\
    \emojibear~Bear  &   0.300    &  {0.564}     &   {0.298}    &    0.565    &   \textbf{0.305}    &   \textbf{0.555}\\
    \emojipig~Pig   &  0.307     &  0.582   &   \textbf{0.308}    &  0.575      &   0.306    &  \textbf{0.596} \\
    \midrule
    Mean   &  \textbf{0.311}     &  0.560   &   {0.308}    &  0.538      &   0.308    &  \textbf{0.562} \\
    \bottomrule
    \end{tabular}%
    }
    % \vspace{-5mm}
    \label{tab:ablation_gan}%
\end{table}%

==> tables/ablation_layer.tex <==
\begin{table}[htbp]
\centering
\caption{We conduct an ablation study using different combinations of losses on layered image editing and report the CLIP score (the higher the better).}
\vspace{3mm}
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{l@{\,}c@{\,}lrrrrr}
\toprule
&&& Text2LIVE & $L_{LSD}$ & $L_{LSD}+L_{KL}$ & $L_{LSD}+L_{FM}$ & $L_{LSD}+L_{KL}+L_{FM}$ \\
\midrule
Horse &$\rightarrow$& Giraffe  & 0.3804  & \textbf{0.3765} & 0.3591  & 0.3445 & 0.3501\\
Horse &$\rightarrow$& Golden horse  & 0.3718  & 0.3503  & \textbf{0.3572} & 0.3440       & 0.3479 \\
Horse &$\rightarrow$& Longmane horse & 0.3547 & 0.2747 & 0.2644 & 0.2710  & \textbf{0.2781} \\
Horse &$\rightarrow$& Zebra & 0.3560  & 0.3337 & 0.3394 & 0.3374 & \textbf{0.3457}\\
Bear  &$\rightarrow$& Pandas & 0.3367& \textbf{0.3145}& 0.3096 & 0.3101 & 0.3022  \\
Bear  &$\rightarrow$& Polar bear  & 0.3206 & \textbf{0.2998}& 0.2915 & 0.2966 & 0.2815\\
Bread &$\rightarrow$& Sandwich& 0.3120& 0.3293& \textbf{0.3359}& 0.3291& 0.3306 \\
Cat   &$\rightarrow$& Tiger & 0.3250  & 0.3169  & \textbf{0.3347} & 0.3201& 0.3262  \\
Black swan &$\rightarrow$& White swan & 0.3037 & 0.2471  & \textbf{0.2467} & 0.2457& 0.2454\\
\midrule
Mean&&& 0.3401  & \textbf{0.3159}& 0.3154 & 0.3109 & 0.3120  \\
\bottomrule
\end{tabular}%
}
\label{tab:ablation_layer}%
\end{table}

==> tables/quantitative_RPrecision_transpose.tex <==
\begin{table}[htbp]
    \centering
    \scriptsize
    \caption{R-Precision: the coherence of our model generations with their caption using different CLIP retrieval models.}
    \begin{tabular}{cccccccc}
    \multirow{2}{*}{Method} & GT & Dream- & CLIP- & Latent & Ours (Latent & Jacobian & Ours (Jacobian \\
     & images & Fields~\cite{jain2021dreamfields} & Mesh~\cite{} & NeRF~\cite{} & NeRF) & NeRF~\cite{} & NeRF) \\
    CLIPB/32 & 77.1 &  &  &  &  &  &  \\
    CLIPB/16 & 79.1 &  &  &  &  &  & 
    \end{tabular}
    \label{tab:quan_RPrecision}
\end{table}
